Improving Video Compression With Deep Visual-Attention Models

Recent advances in deep learning have markedly improved the quality of visual-attention modelling. In this work we apply these advances to video compression. We propose a compression method that uses a saliency model to adaptively compress frame areas in accordance with their predicted saliency. We selected three state-of-the-art saliency models, adapted them for video compression and analyzed their results. The analysis includes objective evaluation of the models as well as objective and subjective evaluation of the compressed videos. Our method, which is based on the x264 video codec, can produce videos with the same visual quality as regular x264, but it reduces the bitrate by 25% according to the objective evaluation and by 17% according to the subjective one. Also, both the subjective and objective evaluations demonstrate that saliency models can compete with gaze maps for a single observer. Our method can extend to most video bitstream formats and can improve video compression quality without requiring a switch to a new video encoding standard.

==> Improving Video Compression With Deep Visual-Attention Models/figures/compression_objective_metrics.tex <==
\begin{figure}[h]
% This file was created by matplotlib2tikz v0.6.18.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{1,0.498039215686275,0.0549019607843137}
\definecolor{color2}{rgb}{0.172549019607843,0.627450980392157,0.172549019607843}
\definecolor{color3}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}
\definecolor{color4}{rgb}{0.580392156862745,0.403921568627451,0.741176470588235}
\definecolor{color5}{rgb}{0.549019607843137,0.337254901960784,0.294117647058824}
\definecolor{color6}{rgb}{0.890196078431372,0.466666666666667,0.76078431372549}
\definecolor{color7}{rgb}{0.737254901960784,0.741176470588235,0.133333333333333}
\definecolor{color8}{rgb}{0.0901960784313725,0.745098039215686,0.811764705882353}

\begin{axis}[
scale only axis,
width={0.84\linewidth},
height={0.9\linewidth},
xlabel={\small Bitrate (kbps)},
%xlabel={\small Битрейт (кбит/с)},
xtick={1000, 1100, 1330, 1500, 1750},
ylabel={\small EWSSIM~\cite{Li2011}},
%ylabel={\small EWSSIM},
legend cell align={left},
legend style={
anchor=south east, 
at={(1,0.0)}, 
fill=white,fill opacity=0.5, draw opacity=1,text opacity=1,
draw=none,
nodes={scale=0.82, transform shape},
font=\small
},
grid=both,
every minor grid/.style={dashed, opacity=0.00},
every major grid/.style={dashed, opacity=0.75},
y tick label style = {rotate=35, anchor=east},
tick align=inside,
tick pos=left,
x grid style={white!69.01960784313725!black},
xmin=1000, xmax=1755,
ymin=0.891, ymax=0.927,
axis x line*=bottom,
axis y line*=left,
y label style={anchor=north east, at={(0.0,0.99)}},
]

\addplot [thick, color0]
table [row sep=\\]{%
996.613569567247	0.906934140742808 \\
1096.89188826581	0.912319740077781 \\
1247.01723666354	0.919079196266946 \\
1497.8639347643	0.927530300254343 \\
1749.52700949242	0.933833279251177 \\
};
\addlegendentry{Ground truth};
%\addlegendentry{Эталонное ВВ};

\addplot [thick, color1]
table [row sep=\\]{%
995.145724225053	0.899910904018229 \\
1095.04121153692	0.905427256240007 \\
1244.73368484249	0.912424430013204 \\
1494.56155021397	0.921086290626344 \\
1745.36484663044	0.927706386432081 \\
};
\addlegendentry{Single observer+PP}
%\addlegendentry{Один зритель+PP}

\addplot [thick, dashed, color2, mark=x]
table [row sep=\\]{%
997.290930644363	0.899081864653934 \\
1097.4388255509	0.904921205903883 \\
1247.6465733835	0.911897693619393 \\
1498.43804257664	0.920879816899288 \\
1749.54091682823	0.927642928275595 \\
};
\addlegendentry{SAM-ResNet+FT+PP}

\addplot [thick, color3]
table [row sep=\\]{%
998.802574437406	0.898137855316835 \\
1098.84298622313	0.903883091332698 \\
1249.20163685858	0.9110241159311 \\
1500.20880895481	0.919949659810052 \\
1751.36874047955	0.926871393266632 \\
};
\addlegendentry{SAM-ResNet+FT}

\addplot [thick, dashed, color4, mark=diamond*]
table [row sep=\\]{%
996.700184487191	0.89753970610526 \\
1096.69222705759	0.903231229632272 \\
1247.14227114829	0.910069593430288 \\
1497.3746408008	0.919109874252358 \\
1748.32376887058	0.925939892859649 \\
};
\addlegendentry{ACL+FT+PP}

\addplot [thick, mark=square*, color=red!50!white]
table [row sep=\\]{%
996.492411175105	0.894414148969645 \\
1096.73212613987	0.900401542336944 \\
1246.32314128101	0.907558917468283 \\
1496.45770794402	0.916914327666043 \\
1746.75977980999	0.923916549253798 \\
};
\addlegendentry{OM-CNN+FT+PP}

\addplot [thick, dashed, color=green!50!black]
table [row sep=\\]{%
999.675520133336	0.894475383242604 \\
1100.3032572018	0.900293765426863 \\
1250.79843172958	0.907730530846382 \\
1502.07384298405	0.916752109091441 \\
1753.49563135161	0.923715448401888 \\
};
\addlegendentry{ACL}

\addplot [thick, white!49.80392156862745!black, mark=o*]
table [row sep=\\]{%
995.135735585462	0.892521069187013 \\
1095.08931369057	0.898497394821583 \\
1244.90097214686	0.905822666893861 \\
1494.30170342638	0.915190558027724 \\
1744.31234040662	0.922364883514201 \\
};
\addlegendentry{Center prior}
%\addlegendentry{Предпочтение центру}

\addplot [thick, color7]
table [row sep=\\]{%
1002.03627215803	0.889735127053242 \\
1102.37023042135	0.895856411074847 \\
1252.4882540838	0.90360489353176 \\
1503.7734038292	0.913292050008313 \\
1755.36383534785	0.920815970343256 \\
};
\addlegendentry{SAM-ResNet}

\addplot [thick, color8, mark=diamond]
table [row sep=\\]{%
995.950469740738	0.881268694671931 \\
1096.2280275556	0.887587612818464 \\
1246.67633442115	0.895650073224137 \\
1497.66370976475	0.905669321237843 \\
1748.45787297905	0.913449162362551 \\
};
\addlegendentry{Regular x264}

% white box
\fill[opacity=0.8, white] (1050.01,0.8992) rectangle (1250,0.8992);

% line
\draw[stealth-stealth,line width=0.75pt, opacity=0.7] (999.269,0.8992) -- (1330,0.8992);

% caption
 \node at (1150,0.8992) [anchor=north, black!75!white] {\fontsize{6.5}{7}\selectfont \textbf{bit-rate savings}};
%\node at (1150,0.8992) [anchor=north, black!75!white] {\fontsize{6.5}{7}\selectfont \textbf{экономия битрейта}};

\end{axis}

\end{tikzpicture}

\vspace{-0.3cm}
\caption{Objective evaluation of proposed saliency-aware compression for different saliency models using the EWSSIM~\cite{Li2011} metric.}
\label{fig:CompressionEWSSIM}
\end{figure}

==> Improving Video Compression With Deep Visual-Attention Models/figures/compression_subjective.tex <==
\begin{figure}[th]

\begin{tikzpicture}
\begin{axis}[
width=\linewidth,
xlabel={\small Bitrate (kbps)},
%xlabel={\small Битрейт (кбит/c)},
ylabel={\small Subjective rank},
%ylabel={\small Субъективная оценка ранга},
xtick={1250, 1375, 1500},
legend cell align={left},
legend style={
anchor=north west, 
at={(0.0,1.0)}, 
fill=white,fill opacity=0.25, draw opacity=1,text opacity=1,
draw=none,
%nodes={scale=0.85, transform shape},
font=\tiny
},
grid=both,
every minor grid/.style={thin, solid, opacity=0.0},
every major grid/.style={thin, solid, opacity=0.5},
%y tick label style = {rotate=35, anchor=east},
tick align=inside,
tick pos=left,
x grid style={white!66!black},
xmin=1240, xmax=1500,
ymin=1.41, ymax=2.57,
axis x line*=bottom,
axis y line*=left,
%y label style={anchor=north east, at={(0.0,0.99)}},
]


\addplot [thick, green!80!black, mark=diamond*, error bars/.cd, y dir=both, y explicit]
plot coordinates {
(1250, 1.8138125049358316) +=(0, 0.191763109529423) -=(0, 0.19176310952942366)
(1375, 2.102174544075585) +=(0, 0.19653250192495397) -=(0, 0.19653250192495286)
(1500, 2.454652033084173) +=(0, 0.212023029985152) -=(0, 0.21202302998515288)
};
\addlegendentry{SAM-ResNet+FT+PP};

\addplot [thick, orange, mark=*]
plot coordinates {
(1250, 1.736000892290858)
(1375, 2.0726369782235747)
(1500, 2.507041849734532)
};
\addlegendentry{Ground truth};

\addplot [thick, gray, mark=square*]
plot coordinates {
(1250, 1.6402800678714964)
(1375, 1.7344220481531183)
(1500, 2.1120790676441503)
};
\addlegendentry{OM-CNN+FT+PP};

\addplot [thick, blue, mark=diamond]
plot coordinates {
(1250, 1.6062935534409908)
(1375, 1.6160258738768682)
(1500, 2.2757746390775813)
};
\addlegendentry{ACL+FT+PP};

\addplot [thick, pink!90!black, mark=*]
plot coordinates {
(1250, 1.4958027381197634)
(1375, 1.6885923412532682)
(1500, 2.0395038303481385)
};
\addlegendentry{Single observer+PP};
%\addlegendentry{Один зритель+PP};

\addplot [thick, purple, mark=o]
plot coordinates {
(1250, 1.4509349190135097)
(1375, 1.5483096302371775)
(1500, 2.172323028595996)
};
\addlegendentry{Center prior};
%\addlegendentry{Предпочтение центру};




\addplot [thick, dashed, red!80!black]
plot coordinates {
    (1000,1.788)
    (2000,1.788)
};
\addlegendentry{Regular x264, 1500 kbps};

\end{axis}
\end{tikzpicture}

\vspace{-0.3cm}
\caption{Subjective evaluation of the proposed saliency-aware compression using different saliency models. 85\% confidence intervals are shown for SAM-ResNet model.}
\label{fig:CompressionSubjective}
\end{figure}

==> Improving Video Compression With Deep Visual-Attention Models/figures/encoder_schema.tex <==
\begin{figure}
    \centering
    \tikzstyle{block} = [draw, fill=white, rectangle, 
        minimum height=3em, minimum width=6em, text width=2cm, align=flush center]
    \tikzstyle{branch} = [fill, shape=circle, minimum size=3pt, inner sep=0pt]
    \tikzstyle{input} = [coordinate]
    \tikzstyle{output} = [coordinate]

    \begin{tikzpicture}[auto, node distance=2cm,>=latex']
        \node [input, name=input] {};
        \node [block, right=2.9cm of input] (encoder) {Encoding module};
        \path (input) -- coordinate (branch) (encoder);
        \node [block, below of=encoder] (saliency) {Saliency prediction module};
        \node [output, name=output, right=2.9cm of encoder] {};
        
        \draw[->] (branch) node[branch] {}{} |- (saliency);
        \draw [->] (input) -- node {Input video} (encoder);
        \draw [->] (saliency) -- (encoder);
        \draw [->] (encoder) -- node {Encoded stream} (output);
    \end{tikzpicture}

    \caption{Scheme of proposed saliency-aware encoder.}
    \label{fig:encoder-schema}
\end{figure}

==> Improving Video Compression With Deep Visual-Attention Models/figures/models_examples.tex <==
\begin{figure*}[!th]
    \begin{center}\small\bfseries\sffamily

    	\newcommand{\contourblack}[1]{\textpdfrender{%
    			StrokeColor = black,
    			TextRenderingMode=FillStroke,
    			FillColor=yellow,
    			LineWidth=.07ex,
    		}{#1}
    	}

        \setlength{\tabcolsep}{1pt}
        \renewcommand{\arraystretch}{1}

        \begin{tabular}[h!]{p{0.24\linewidth}p{0.24\linewidth}p{0.24\linewidth}p{0.24\linewidth}}

            \begin{mtikzonimage}{\linewidth}{models_examples/frames.jpg}
                \node[color=yellow, left=2pt] at (\linewidth, 0.5\baselineskip) {\fontsize{7pt}{7pt}\selectfont Source Frame};
            \end{mtikzonimage}\stepcounter{mcounter} &

            \begin{mtikzonimage}{\linewidth}{models_examples/gt_saliency_rad=90_max_nrm.jpg}
                \node[color=yellow, left=2pt] at (\linewidth, 0.5\baselineskip) {\fontsize{7pt}{7pt}\selectfont Ground-truth};
            \end{mtikzonimage}\stepcounter{mcounter} &
            
            \begin{mtikzonimage}{\linewidth}{models_examples/CP.jpg}
                \node[color=yellow, left=2pt] at (\linewidth, 0.5\baselineskip) {\fontsize{7pt}{7pt}\selectfont Center prior};
            \end{mtikzonimage}\stepcounter{mcounter}&
        
            \begin{cropimg}{\linewidth}{models_examples/saliency_single-observer-postprocessed-gt-rad-120}
                      {0.35\linewidth}{models_examples/saliency_single-observer}
                \node[color=yellow, left=2pt] at (\linewidth, 0.5\baselineskip) {\fontsize{7pt}{7pt}\selectfont Single Observer};
            \end{cropimg}\stepcounter{mcounter}
            
        \tabularnewline[-0.4cm]
            
            &
        
            \begin{cropimg}{\linewidth}{models_examples/saliency_OM-CNN-4-datasets-postprocessed-gt-rad-120}
                     {0.35\linewidth}{models_examples/saliency_OM-CNN-4-datasets}
                \node[color=yellow, left=2pt] at (\linewidth, 0.5\baselineskip) {\fontsize{7pt}{7pt}\selectfont OM-CNN~\cite{OM-CNN-Jiang2017}};
            \end{cropimg}\stepcounter{mcounter} &

            \begin{cropimg}{\linewidth}{models_examples/saliency_acl_fine-tuned_best-loss-postprocessed-gt-rad-120}
                     {0.35\linewidth}{models_examples/saliency_acl_vanilla}
                \node[color=yellow, left=2pt] at (\linewidth, 0.5\baselineskip) {\fontsize{7pt}{7pt}\selectfont ACL~\cite{ACL-wang2018}};
            \end{cropimg}\stepcounter{mcounter} &
            
            \begin{cropimg}{\linewidth}{models_examples/saliency_sam-resnet_ft-cc-only-loss-best-postprocessed-gt-rad-120}
                     {0.35\linewidth}{models_examples/saliency_sam-resnet_original-resnet}
                \node[color=yellow, left=2pt] at (\linewidth, 0.5\baselineskip) {\fontsize{7pt}{7pt}\selectfont SAM-ResNet~\cite{SAM-cornia2018}};
            \end{cropimg}\stepcounter{mcounter}
            
        \end{tabular}
    \end{center}
    
    \vspace{-0.6cm}
    \caption{%
    	Saliency maps for three selected models and baselines.
    	Fine-tuned and postprocessed saliency maps of the models are shown.
    	Also, original saliency maps are shown in the left bottom corner of the image.
%    	Histograms of all images are normalized for visibility.
%    	For each model its original, fine-tuned and postprocessed versions are provided.
    }\label{fig:ModelExamples}
	
	\vspace{-0.45cm}
	
\end{figure*}

==> Improving Video Compression With Deep Visual-Attention Models/figures/saliency_objective_metrics.tex <==
\begin{table}[!t]

\centering
\resizebox{\linewidth}{!}{%
\begin{tabular}{lccccc}
\toprule
Model &  AUC-J$\uparrow$ &     CC$\uparrow$ &  KL$\downarrow$ &    NSS$\uparrow$ &  SIM$\uparrow$ \\
\midrule
\scriptsize Ground truth         &     -     &  -     &  -      &  3.250 & - \\
\scriptsize SAM-ResNet + FT + PP &     0.833 &  0.672 &   0.569 &  2.021 &             0.618 \\
\scriptsize SAM-ResNet + FT      &     0.835 &  0.664 &   1.242 &  2.180 &             0.616 \\
\scriptsize Single observer + PP &     0.807 &  0.651 &   0.621 &  1.845 &             0.603 \\
\scriptsize ACL + FT + PP        &     0.820 &  0.633 &   0.584 &  1.705 &             0.603 \\
\scriptsize ACL + FT             &     0.820 &  0.631 &   0.651 &  1.764 &             0.604 \\
\scriptsize Single observer      &     0.763 &  0.581 &   9.601 &  2.465 &             0.493 \\
\scriptsize OM-CNN + FT          &     0.791 &  0.560 &   0.863 &  1.504 &             0.569 \\
\scriptsize OM-CNN + FT + PP     &     0.790 &  0.557 &   0.691 &  1.417 &             0.563 \\
\scriptsize OM-CNN               &     0.781 &  0.553 &   1.652 &  1.462 &             0.560 \\
\scriptsize ACL                  &     0.796 &  0.552 &   1.985 &  1.769 &             0.546 \\
\scriptsize SAM-ResNet           &     0.842 &  0.543 &   2.818 &  2.220 &             0.517 \\
\scriptsize Center prior         &     0.751 &  0.469 &   1.731 &  1.087 &             0.503 \\
\bottomrule
\end{tabular}
}

\caption{Objective evaluation results of the selected models and the baselines using five metrics on the SAVAM~\cite{Gitman2014} dataset. The results include the original models, the fine-tuned models for the training part of the SAVAM dataset (FT), and the result after applying the postprocessing transformations (PP).}
\label{tab:SaliencyObjectiveMetrics}

\end{table}
